aiXcoder-7B: A Lightweight and Effective Large Language Model for Code Processing

Large Language Models (LLMs) have been widely used in code completion, and researchers are focusing on scaling up LLMs to improve their accuracy. However, larger LLMs have lower inference efficiency, affecting developers' experience and productivity. In this paper, we propose a lightweight and effective LLM for code completion named aiXcoder-7B. Compared to existing LLMs, aiXcoder-7B achieves higher code completion accuracy while having smaller scales (i.e., 7 billion parameters). We attribute the superiority of aiXcoder-7B to three key factors: (1) Multi-objective training. We employ three training objectives, one of which is our proposed Structured Fill-In-the-Middle (SFIM). SFIM considers the syntax structures in code and effectively improves the performance of LLMs for code. (2) Diverse data sampling strategies. They consider inter-file relationships and enhance the capability of LLMs in understanding cross-file contexts. (3) Extensive high-quality data. We establish a rigorous data collection pipeline and consume a total of 1.2 trillion unique tokens for training aiXcoder-7B. This vast volume of data enables aiXcoder-7B to learn a broad distribution of code. We evaluate aiXcoder-7B in five popular code completion benchmarks and a new benchmark collected by this paper. The results show that aiXcoder-7B outperforms the latest six LLMs with similar sizes and even surpasses four larger LLMs (e.g., StarCoder2-15B and CodeLlama-34B), positioning aiXcoder-7B as a lightweight and effective LLM for academia and industry. Finally, we summarize three valuable insights for helping practitioners train the next generations of LLMs for code. aiXcoder-7B has been open-souced and gained significant attention. Until January 2025, aiXcoder-7B has received 2,226 GitHub Stars.

==> table/extend_data_1.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\centering
\caption{Details of different models evaluation results on the Java programming language}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccccc}
\midrule
 \multirow{3}{*}{\textbf{aiXcoder-7B-Base}}  & \multicolumn{5}{c}{\textbf{Java}} \\  \cmidrule{2-8}
 & \multicolumn{1}{c}{\textbf{EM(\%)}} & \multicolumn{1}{c}{\textbf{BLEU-4}} & \multicolumn{1}{c}{\textbf{CodeBLEU}} & \multicolumn{1}{c}{\textbf{Length(Pred/Ref)}} & \multicolumn{1}{c}{\textbf{Case Number}}&& \\
\midrule 
method signature&65.3&82.0&89.3&60/62&600 \\
method body&48.1&69.7&76.5&142/139&600 \\
single line&78.6&84.3&81.5&53/22&600 \\
method with comment&44.5&72.9&80.8&184/157&600 \\
empty&95.0&95.0&48.7&17/0&180 \\
method body top&40.0&59.9&65.1&206/228&200 \\
method body mid &31.5&57.5&65.1&319/492&200 \\
method body bottom&56.0&68.7&65.5&196/290&200 \\
if statement&37.7&60.8&70.8&182/160&180 \\
for statement&19.4&61.0&67.0&304/221&180 \\
while statement &17.7&58.6&65.4&226/231&180 \\
try statement&15.5&50.8&59.9&219/266&180 \\
switch case&5.5&38.7&53.1&271/330&180 \\
Total&49.4&70.6&74.0&154/159&4080 \\
\midrule
\\
\midrule
\multirow{1}{*}{\textbf{DeepSeekCoder-7B}}  && \\
\midrule
method signature&61.5&76.9&88.3&97/62&600 \\
method body&41.0&60.8&73.6&234/139&600 \\
single line&70.1&76.5&79.5&94/22&600 \\
method with comment&34.3&59.6&76.9&301/157&600 \\
empty&82.2&82.2&45.6&66/0&180 \\
method body top&47.0&68.2&67.0&170/228&200 \\
method body mid &23.5&51.5&62.2&330/492&200 \\
method body bottom&51.0&62.7&65.0&252/290&200 \\
if statement&31.1&54.7&67.2&216/160&180 \\
for statement&17.2&53.5&63.6&318/221&180 \\
while statement &13.3&50.1&61.2&321/231&180 \\
try statement&12.7&44.7&57.5&331/266&180 \\
switch case&3.8&37.6&53.7&407/330&180 \\
Total&43.4&63.4&71.7&217/159&4080 \\
\bottomrule
\end{tabular}
}

\label{tab:extent_data_1}
\end{table}

==> table/extend_data_2.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\centering
\caption{Details of different models evaluation results on the Python programming language }
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccccc}
\midrule
 \multirow{1}{*}{\textbf{aiXcoder-7B-Base}}  & \multicolumn{5}{c}{\textbf{Python}} \\  \cmidrule{2-8}
 & \multicolumn{1}{c}{\textbf{Exact Match(\%)}} & \multicolumn{1}{c}{\textbf{BLEU-4}} & \multicolumn{1}{c}{\textbf{CodeBLEU}} & \multicolumn{1}{c}{\textbf{Length(Pred/Ref)}} & \multicolumn{1}{c}{\textbf{Case Number}}&& \\
\midrule 
method signature&51.0&69.9&81.9&107/41&600 \\
method body&20.1&41.4&54.0&147/186&600 \\
single line&69.1&76.8&75.8&59/19&600 \\
method with comment&23.5&52.1&61.2&207/199&600 \\
empty&95.0&95.0&48.7&15/0&180 \\
method body top&10.5&34.4&50.3&131/308&200 \\
method body mid &19.0&47.3&59.4&233/280&200 \\
method body bottom&22.5&49.4&57.6&263/673&200 \\
if statement&26.1&49.9&62.6&157/144&180 \\
for statement&17.7&47.3&56.2&189/179&180 \\
while statement &10.0&43.1&53.0&204/218&180 \\
try statement&7.2&34.7&49.8&153/202&180 \\
Total&35.0&56.1&63.0&146/167&3900 \\
\midrule
\\
\midrule
\multirow{1}{*}{\textbf{DeepSeekCoder-7B}}  && \\
\midrule
method signature&51.8&70.3&83.3&125/41&600 \\
method body&14.3&40.2&58.2&362/186&600 \\
single line&53.3&60.4&71.7&173/19&600 \\
method with comment&14.0&40.2&58.9&420/199&600 \\
empty&85.0&85.0&46.3&69/0&180 \\
method body top&12.5&48.2&60.9&301/308&200 \\
method body mid &22.0&50.1&62.2&292/280&200 \\
method body bottom&17.5&44.3&57.5&411/673&200 \\
if statement&27.2&51.2&65.5&235/144&180 \\
for statement&13.3&39.0&54.4&336/179&180 \\
while statement &7.7&37.6&51.4&344/218&180 \\
try statement&6.1&32.8&49.4&256/202&180 \\
Total&29.6&51.1&63.4&275/167&3900 \\
\bottomrule
\end{tabular}
}

\label{tab:extent_data_2}
\end{table}

==> table/extend_data_3.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\centering
\caption{Details of different models evaluation results on the C++ programming language }
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccccc}
\midrule
 \multirow{1}{*}{\textbf{aiXcoder-7B-Base}}  & \multicolumn{5}{c}{\textbf{C++}} \\  \cmidrule{2-8}
 & \multicolumn{1}{c}{\textbf{Exact Match(\%)}} & \multicolumn{1}{c}{\textbf{BLEU-4}} & \multicolumn{1}{c}{\textbf{CodeBLEU}} & \multicolumn{1}{c}{\textbf{Length(Pred/Ref)}} & \multicolumn{1}{c}{\textbf{Case Number}}&& \\
\midrule  
method signature&53.6&72.2&82.0&83/64&600 \\
method body&31.0&57.7&65.2&199/164&600 \\
single line&70.6&76.9&80.0&78/18&600 \\
method with comment&13.1&45.7&6.0&349/214&600 \\
empty&89.4&89.4&47.4&31/0&180 \\
method body top&33.0&55.4&65.4&274/166&200 \\
method body mid &23.0&52.5&64.6&372/422&200 \\
method body bottom&44.0&63.8&67.0&374/302&200 \\
if statement&29.4&57.1&68.9&202/141&180 \\
for statement&19.4&58.1&65.5&261/201&180 \\
while statement &12.7&51.6&60.9&241/210&180 \\
try statement&12.2&37.0&52.3&264/256&180 \\
switch case&11.1&41.7&56.5&421/314&180 \\
Total&37.3&60.3&67.4&217/161&4080 \\
\midrule
\\
\midrule
\multirow{1}{*}{\textbf{DeepSeekCoder-7B}}  && \\
\midrule
method signature&49.1&67.5&81.8&180/64&600 \\
method body&18.6&41.7&61.8&388/164&600 \\
single line&57.3&63.0&76.4&175/18&600 \\
method with comment&9.5&35.4&59.6&512/214&600 \\
empty&73.3&73.3&43.6&146/0&180 \\
method body top&27.5&54.6&67.7&282/166&200 \\
method body mid &17.5&48.8&63.8&382/422&200 \\
method body bottom&29.0&47.3&64.3&382/302&200 \\
if statement&21.1&48.7&68.3&305/141&180 \\
for statement&10.5&45.3&63.4&373/201&180 \\
while statement &9.4&43.1&59.9&372/210&180 \\
try statement&8.8&32.4&54.3&414/256&180 \\
switch case&5.5&30.5&52.7&521/314&180 \\
Total&29.1&50.0&65.8&330/161&4080 \\
\bottomrule
\end{tabular}
}

\label{tab:extent_data_3}
\end{table}

==> table/extend_data_4.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{3pt}
\centering
\caption{Details of different models evaluation results on the JavaScript programming language }
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccccccc}

\midrule
 \multirow{1}{*}{\textbf{aiXcoder-7B-Base}}  & \multicolumn{5}{c}{\textbf{JavaScript}} \\  \cmidrule{2-8}
 & \multicolumn{1}{c}{\textbf{Exact Match(\%)}} & \multicolumn{1}{c}{\textbf{BLEU-4}} & \multicolumn{1}{c}{\textbf{CodeBLEU}} & \multicolumn{1}{c}{\textbf{Length(Pred/Ref)}} & \multicolumn{1}{c}{\textbf{Case Number}}&& \\
\midrule 
method signature&72.5&80.6&88.2&45/32&600 \\
method body&16.1&46.2&57.0&191/182&600 \\
single line&65.5&74.3&75.9&48/19&600 \\
method with comment&12.0&43.9&56.7&293/209&600 \\
empty&97.2&97.2&49.3&46/0&180 \\
method body top&26.0&46.3&55.7&196/199&200 \\
method body mid &9.5&41.7&53.5&305/492&200 \\
method body bottom&52.0&64.6&59.3&124/536&200 \\
if statement&17.2&44.5&60.8&230/136&180 \\
for statement&23.3&61.5&66.2&217/187&180 \\
while statement &23.8&54.8&64.1&228/173&180 \\
try statement&8.8&35.7&51.1&244/213&180 \\
switch case&6.6&34.8&52.1&438/303&180 \\
Total&36.5&58.0&64.3&177/170&4080 \\
\midrule
\\
\midrule
\multirow{1}{*}{\textbf{DeepSeekCoder-7B}}  && \\
\midrule
method signature&61.1&69.7&84.0&106/32&600 \\
method body&10.6&36.7&52.7&246/182&600 \\
single line&57.3&65.9&72.6&101/19&600 \\
method with comment&7.0&36.2&53.5&336/209&600 \\
empty&82.2&82.2&45.6&81/0&180 \\
method body top&29.5&50.6&57.2&174/199&200 \\
method body mid &7.5&39.2&51.0&317/492&200 \\
method body bottom&42.5&56.8&57.4&252/536&200 \\
if statement&11.6&37.2&57.5&242/136&180 \\
for statement&15.0&46.9&57.5&300/187&180 \\
while statement &8.3&35.3&53.2&390/173&180 \\
try statement&3.8&26.0&46.0&319/213&180 \\
switch case&2.2&24.7&47.3&471/303&180 \\
Total&29.3&49.0&60.3&232/170&4080 \\
\bottomrule
\end{tabular}
}

\label{tab:extent_data_4}
\end{table}
